Handling Communication via APIs for Microservices

Enterprises in their journey to the cloud, want to decompose their monolith applications into microservices to maximize cloud benefits. Current research focuses a lot on how to partition the monolith into smaller clusters that perform well across standard metrics like coupling, cohesion, etc. However, there is little research done on taking the partitions, identifying their dependencies between the microservices, exploring ways to further reduce the dependencies, and making appropriate code changes to enable robust communication without modifying the application behaviour. In this work, we discuss the challenges with the conventional techniques of communication using JSON and propose an alternative way of ID-passing via APIs. We also devise an algorithm to reduce the number of APIs. For this, we construct subgraphs of methods and their associated variables in each class and relocate them to their more functionally aligned microservices. Our quantitative and qualitative studies on five public Java applications clearly demonstrate that our refactored microservices using ID have decidedly better time and memory complexities than JSON. Our automation reduces 40-60\% of the manual refactoring efforts.

==> Sections/comments.tex <==
Figure 2:
1. Step[3] : Identify methods called by another cluster -> Identify methods called by other clusters. 
%suggesting this because the api candidates must be called by more than one clusters excluding its own.
2. Either the caption should be made "steps 0-4" or or figure must change to 1-5 for consistency.
3. I could not find the step 5 (or step 4 according to the numbering in the figure). 
4. Just a suggestion: the width of the grey arrows can make this figure look more comprehensive and put together.
5. Adding terminator (a full stop) after each point and justifying their alignments will also look better.




==> Sections/decouplingErrors.tex <==
1. Missing dependent jars + undefined annotations
import javax.xml.parsers.DocumentBuilderFactory;
@Entity
2. Direct creation of a class' object
private static TradeServices tradeRemote = null;
3. Direct access to other class' field member

4. Return type/ argument type as some other class


% Proving semantic equivalence of two program is an undecidable problem. 

==> Sections/socc-rebuttal.tex <==
\renewcommand{\thesubsection}{\arabic{subsection}.}

\section*{SoCC'22 Rebuttal}

\subsection{Motivation: Monolith to Microservices}
 We agree with the reviewer's observation that sometimes it is easier to build microservices from scratch rather than refactoring the monolith. However, this requires the developers to have a sufficient understanding of the monolith's implementation details and expertise in building microservices. From our discussions with the developers and prior arts, there seems to be substantial merit in automatically enabling microservices, even if their performance may not be at par with the ones written from scratch. This way, the developers can focus on optimizing performance bottlenecks (e.g, transaction management like SAGA) rather than worrying if they had covered all the original use cases.
({\bf \textcolor{red}{Reviewer\#51E}})

\subsection{Technical Contributions}
({\bf\textcolor{red}{Reviewer\#51B, \#51D}})
\begin{itemize}
\item ID-passing approach: Section 5
\item Refactoring in the least intrusive way: Section 5.1 (Wrapper approach)
\item Reducing data communication: Section 6
\item Creating more functionally aligned microservices: Section 6
\end{itemize}

\subsection{ID-Passing vs. JSON-Passing Performance}

End of Section 5.2 already has some comparisons (including performance). We elaborate these below. ({\bf\textcolor{red}{Reviewer\#51A, \#51C, \#51D}})

\subsubsection{Advantages of ID-Passing}

\begin{enumerate}
\item 
The ID-passing approach preserves the semantics of the application.
\item 
Less memory wastage: Objects are created and sustained only on the server-side; they are not duplicated on the client-side.
\item 
More efficient, better readability, and less refactoring of monolith: In API call, JSON-passing requires merging parameters and serialization; API return requires deserialization and unmerging of parameters. On the caller side, any changes made to the objects need to be updated. All these are not required in the ID-passing approach as it passes only IDs of the objects.
\item 
It may be more efficient than JSON passing as it does not require serialization and deserialization. The complexity of JSON serialization is O(|N| x complexity of depth-first search), i.e., O(|N| x (|N| + |E|)) because values of all the pointers for each path in a graph data structure are serialized. In comparison, the complexity of ID-passing is O(1) since only ID needs to be passed.

\item 
Good data distribution: It saves objects in the memory of the microservice that owns it. However, the JSON-passing approach saves all objects in the memory of the microservice that contains the “main(.)” method. Thereby making one microservice a hotspot, which is not the case in the ID-passing approach. ({\bf\textcolor{red}{Reviewer\#51A}})
\\
For example: let us see how data is saved in JSON-passing approach: say the monolith has classes A and B, which are split into microservices 1 and 2 containing classes A and B, respectively. Class A contains the pointer objB to object of class B. Class A also contains the main(.) method, which calls API createB() of microservice 2. When microservice 1 starts, the object of class A gets created in microservice 1. API createB() of microservice 2 creates an object of class B, serializes it, sends it to microservice 1, and deletes it from microservice 2. Microservice 1 deserializes it and saves it as objB. Therefore, in JSON-passing, although class B is owned by microservice 2, its instance/object is saved in microservice 1 only. Similarly, all other classes will be saved in microservice 1 only. Therefore, in JSON-passing, data distribution is poor.
\item 
Central DB vs. distributed data on microservices: Some microservice architectures save all objects in a central DB, which are accessed by microservices via object IDs. The disadvantage of this approach is that it is slow due to DB accesses, exposes data between microservices, and makes DB a hotspot. On the other hand, in the ID-passing approach, data is distributed and private with the respective microservice, and faster than DB access.
\end{enumerate}

\subsubsection{Disadvantages of ID-Passing}

\begin{enumerate}
\item
REST API communication generally happens using JSON; use of ID instead of JSON is unconventional.
\item
Leads to more API calls as the server needs to be accessed for any operation on the object created by the server. Depending on the data structures, if an application leads to too many API calls, a developer may use the following design in ID-passing approach: keep local copies of the data in all microservices, update them locally, and restore the updates in the owning microservice periodically using their IDs. ({\bf\textcolor{red}{Reviewer\#51E}})
\end{enumerate}

\subsection{Comparison with Existing Literature}

\begin{itemize}
\item 
References [19, 24]: These only provide information about microservice clusters; they neither construct the microservices nor handle their communication, which is handled in our work. ({\bf\textcolor{red}{Reviewer\#51A}})
\item
State sharding work: Their bottleneck to scalability is storage. Moreover, they lead to duplication of data and require synchronization. These problems do not exist in our work. ({\bf\textcolor{red}{Reviewer\#51B}})
\item 
Microservices Petclinic (Section 9.3): IDs used by microservices Petclinic (Section 9.3) are different from our IDs. This is explained in the paper as follows: Monolith Petclinic already contains IDs to Database objects. On the other hand, we automatically introduce IDs to microservice memory since they may not always be present in the monolith. We save objects in the memory of the microservice, which is better than saving in the central Database (as done by microservices Petclinic). It is better because it is not exposed to all microservices and is faster than Database access. ({\bf\textcolor{red}{Reviewer\#51D}})
\end{itemize}

\newpage

